Exponential Weights on the Hypercube in Polynomial Time

We study a general online linear optimization problem(OLO). At each round, a subset of objects from a fixed universe of $n$ objects is chosen, and a linear cost associated with the chosen subset is incurred. To measure the performance of our algorithms, we use the notion of regret which is the difference between the total cost incurred over all iterations and the cost of the best fixed subset in hindsight. We consider Full Information and Bandit feedback for this problem. This problem is equivalent to OLO on the $\{0,1\}^n$ hypercube. The Exp2 algorithm and its bandit variant are commonly used strategies for this problem. It was previously unknown if it is possible to run Exp2 on the hypercube in polynomial time. In this paper, we present a polynomial time algorithm called PolyExp for OLO on the hypercube. We show that our algorithm is equivalent Exp2 on $\{0,1\}^n$, Online Mirror Descent(OMD), Follow The Regularized Leader(FTRL) and Follow The Perturbed Leader(FTPL) algorithms. We show PolyExp achieves expected regret bound that is a factor of $\sqrt{n}$ better than Exp2 in the full information setting under $L_\infty$ adversarial losses. Because of the equivalence of these algorithms, this implies an improvement on Exp2's regret bound in full information. We also show matching regret lower bounds. Finally, we show how to use PolyExp on the $\{-1,+1\}^n$ hypercube, solving an open problem in Bubeck et al (COLT 2012).

==> suppliment.tex <==
\section{Supplementary Proofs}
\subsection{Exp2 Regret Proofs}
First, we directly analyze Exp2's regret for the two kinds of feedback.
\subsubsection{Full Information}
\begin{lemma}\label{Lemma1}Let $L_t(X) = X^\top l_t$. If $|\eta L_t(X)| \leq 1$ for all $t \in [T]$ and $X \in \{0,1\}^n$, the Exp2 algorithm satisfies for any $X$:
$$\sum_{t=1}^T p_t^\top L_t - \sum_{t=1}^T L_t(X) \leq \eta \sum_{t=1}^T p_t^\top L_t^2 + \frac{n\log 2}{\eta}$$
\end{lemma}
\begin{proof}
(Adapted from \cite{hazan2016introduction} Theorem 1.5) Let $Z_{t} = \sum_{Y \in \{0,1\}^n}w_t(Y)$. We have:
\begin{align*}
Z_{t+1} &= \sum_{Y \in \{0,1\}^n}\exp(-\eta L_t(Y))w_t(Y)\\
&= Z_t \sum_{Y \in \{0,1\}^n}\exp(-\eta L_t(Y)) p_t(Y)
\end{align*}
Since $e^{-x} \leq 1-x+x^2$ for $x\geq -1$, we have that $\exp(-\eta L_t(Y)) \leq 1-\eta L_t(Y)+\eta^2 L_t(Y)^2$ (Because we assume $|\eta L_t(X)| \leq 1$). So,
\begin{align*}
Z_{t+1} &\leq Z_t \sum_{Y \in \{0,1\}^n}(1-\eta L_t(Y)+\eta^2 L_t(Y)^2) p_t(Y) \\
&= Z_t (1 - \eta p_t^\top L_t + \eta^2 p_t^\top L_t^2)
\end{align*}
Using the inequality $1+x \leq e^x$,
\begin{align*}
Z_{t+1} &\leq Z_t \exp( -\eta p_t^\top L_t + \eta^2 p_t^\top L_t^2)
\end{align*}
Hence, we have:
$$Z_{T+1} \leq Z_1 \exp( -\sum_{t=1}^T\eta p_t^\top L_t + \sum_{t=1}^T\eta^2 p_t^\top L_t^2)$$
For any $X \in \{0,1\}^n$, $w_{T+1}(X) = \exp(-\sum_{t=1}^T\eta L_t(X) )$. Since $w(T+1)(X) \leq Z_{T+1}$ and $Z_1 = 2^n$, we have:
\begin{align*}
\exp(-\sum_{t=1}^T\eta L_t(X) ) \leq 2^n \exp( -\sum_{t=1}^T\eta p_t^\top L_t + \sum_{t=1}^T\eta^2 p_t^\top L_t^2)
\end{align*}
Taking the logarithm on both sides manipulating this inequality, we get:
$$\sum_{t=1}^T p_t^\top L_t - \sum_{t=1}^T L_t(X) \leq \eta \sum_{t=1}^T p_t^\top L_t^2 + \frac{n\log 2}{\eta}$$
\end{proof}
\ExpFReg*
\begin{proof}
Using $L_t(X) = X^\top l_t$ and applying expectation with respect to the randomness of the player to definition of regret, we get:
\begin{align*}
E[\mathcal{R}_T] &= \sum_{t=1}^T \sum_{X \in \{0,1\}^n}p_t(X)L_t(X) - \min_{X^\star \in \{0,1\}^n}\sum_{t=1}^T L_t(X^\star) \\
&=  \sum_{t=1}^T p_t^\top L_t - \min_{X^\star \in \{0,1\}^n}\sum_{t=1}^T L_t(X^\star)
\end{align*}
Applying Lemma \ref{Lemma1}, we get $E[\mathcal{R}_T] \leq \eta \sum_{t=1}^T p_t^\top L_t^2 + n\log 2/\eta$. Since $|L_t(X)| \leq n $ for all $X  \in \{0,1\}^n$, we get $\sum_{t=1}^T p_t^\top L_t^2 \leq  T n^2 $.
$$E[\mathcal{R}_T] \leq \eta Tn^2 + \frac{n\log 2}{\eta}$$
Optimizing over the choice of $\eta$, we get the regret is bounded by $2n^{3/2} \sqrt{T \log 2}$ if we choose $\eta = \sqrt{\frac{\log 2}{nT}}$.

To apply Lemma \ref{Lemma1}, $|\eta L_t(X)| \leq 1$ for all $t \in [T]$ and $X \in \{0,1\}^n$. Since $|L_t(X)| \leq n$, we have $\eta \leq 1/n$.
\end{proof}
\subsubsection{Bandit}
\begin{lemma}\label{lemma5_1} Let $\tilde{L_t}(X) = X^\top \tilde{l}_t$, where $\tilde{l}_t = P_t^{-1}X_tX_t^\top l_t$. If $|\eta\tilde{L_t}(X)| \leq 1$ for all $t \in [T]$ and $X \in \{0,1\}^n$, the Exp2 algorithm with uniform exploration satisfies for any $X$
$$\sum_{t=1}^T  q_t^\top L_t - \sum_{t=1}^T L_t(X) \leq \eta \mathbb{E}[\sum_{t=1}^T q_t^\top \tilde{L}_t^2] + \frac{n\log 2}{\eta} + 2\gamma n T$$
\end{lemma}
\begin{proof}
We have that:
\begin{align*}
\sum_{t=1}^T q_t^\top \tilde{L}_t - \sum_{t=1}^T \tilde{L}_t(X)  &= (1-\gamma) (\sum_{t=1}^T p_t^\top \tilde{L}_t - \sum_{t=1}^T \tilde{L}_t(X)) \\&+ \gamma (\sum_{t=1}^T \mu^\top \tilde{L}_t - \sum_{t=1}^T \tilde{L}_t(X))
\end{align*}
Since the algorithm essentially runs Exp2 using the losses $\tilde{L}_t(X)$ and $|\eta\tilde{L_t}(X)| \leq 1$, we can apply Lemma \ref{Lemma1}:
\begin{align*}
\sum_{t=1}^T q_t^\top \tilde{L}_t - \sum_{t=1}^T \tilde{L}_t(X)  &\leq (1-\gamma) (\frac{n \log 2}{\eta} + \eta \sum_{t=1}^T p_t^\top \tilde{L}_t^2) \\&+ \gamma (\sum_{t=1}^T \mu^\top \tilde{L}_t - \sum_{t=1}^T \tilde{L}_t(X))
\end{align*}
Apply expectation with respect to $X_t$.  Using the fact that $\mathbb{E}[\tilde{l}_t] = l_t$ and $\mu^\top L_t -  L_t(X) \leq 2n$:
\begin{align*}
\sum_{t=1}^T q_t^\top L_t - \sum_{t=1}^T L_t(X)  &\leq (1-\gamma) (\frac{n \log 2}{\eta} + \eta \mathbb{E}[\sum_{t=1}^T p_t^\top \tilde{L}_t^2]) \\&+ \gamma (\sum_{t=1}^T \mu^\top L_t - \sum_{t=1}^T L_t(X))\\
&\leq \eta \mathbb{E}[\sum_{t=1}^T q_t^\top \tilde{L}_t^2] + \frac{n \log 2}{\eta}  + 2 \gamma nT
\end{align*}
\end{proof}
\ExpBanReg*
\begin{proof}
Applying expectation with respect to the randomness of the player to the definition of regret, we get:
\begin{align*}
\mathbb{E}[\mathcal{R}_T] &= \mathbb{E}[\sum_{t=1}^T L_t(X_t) - \min_{X^\star \in \{0,1\}^n} L_t(X^\star)] \\&= \sum_{t=1}^T  q_t^\top L_t - \min_{X^\star \in \{0,1\}^n}\sum_{t=1}^T L_t(X^\star)
\end{align*}
Applying Lemma \ref{lemma5_1}
$$\mathbb{E}[\mathcal{R}_T] \leq \eta \mathbb{E}[\sum_{t=1}^T q_t^\top \tilde{L}_t^2] + \frac{n \log 2}{\eta}  + 2 \gamma nT$$
We follow the proof technique of \cite{bubeck2012towards} Theorem 4. We have that:
\begin{align*}
q_t^\top \tilde{L}_t^2 &= \sum_{X \in \{0,1\}^n}q_t(X)(X^\top \tilde{l_t})^2  \\&= \sum_{X \in \{0,1\}^n}q_t(X)(\tilde{l_t}^\top X X^\top \tilde{l_t})\\
&= \tilde{l_t}^\top P_t \tilde{l_t} \\&= l_t^\top X_tX_t^\top P_t^{-1}  P_t P_t^{-1}X_t X_t^\top l_t \\&= (X_t^\top l_t)^2 X_t^\top P_t^{-1}X_t\\
&\leq n^2 X_t^\top P_t^{-1}X_t = n^2 \text{Tr}(P_t^{-1} X_t X_t^\top )
\end{align*}
Taking expectation, we get $E[q_t^\top \tilde{L}_t^2] \leq n^2 \text{Tr}(P_t^{-1} \mathbb{E}[X_t X_t^\top] )= n^2 \text{Tr}(P_t^{-1} P_t) = n^3$.
Hence,
$$\mathbb{E}[\mathcal{R}_T] \leq \eta n^3 T + \frac{n \log 2}{\eta}  + 2 \gamma nT$$
However, in order to apply Lemma \ref{lemma5_1}, we need that $|\eta X^\top \tilde{l}_t| \leq 1$. We have that
$$|\eta X^\top \tilde{l}_t| = \eta |(X_t ^\top l_t) X^\top P_t^{-1} X_t| \leq 1$$
As $|X_t ^\top l_t| \leq n$ and $|X_t^\top X|\leq n$, we get $\eta n |X^\top P_t^{-1} X_t|  \leq \eta n |X^\top X_t|\|P_t^{-1}\|\leq \eta n^2\|P_t^{-1}\| \leq 1 $. The matrix $P_t = (1-\gamma)\Sigma_t + \gamma \Sigma_\mu$. The smallest eigenvalue of $\Sigma_\mu$ is $1/4$\cite{cesa2012combinatorial}. So $P_t \succeq \frac{\gamma}{4} I_n $ and $P_t^{-1} \preceq \frac{4}{\gamma}I_n$. We should have that $\frac{4n^2 \eta}{\gamma}\leq 1$. Substituting $\gamma = 4n^2 \eta$ in the regret inequality, we get:
\begin{align*}
\mathbb{E}[\mathcal{R}_T] &\leq \eta n^3 T + 8\eta n^3 T +  \frac{n \log 2}{\eta}\\
&\leq 9\eta n^3T +  \frac{n \log 2}{\eta}
\end{align*}
Optimizing over the choice of $\eta$, we get $\mathbb{E}[\mathcal{R}_T] \leq 2 n^{2} \sqrt{9T \log 2}$ when $\eta = \sqrt{\frac{\log 2}{9n^2T}}$.
\end{proof}

\subsection{Lower Bounds}
\subsubsection{Full Information Lower bound}


In the game between player and adversary, the players strategy is to pick some probability distribution $p_t \in \Delta(\{0,1\}^n)$ for $t=1\dots T$. The adversary picks a density $q_t$ over loss vectors $l \in [-1,1]^n$ for $t=1 \dots T$. So player picks $X_t \sim p_t$ and adversary picks $l_t \sim q_t$.  The min max expected regret is:
$$\inf_{p_1 \dots p_T} \sup_{q_1 \dots q_t}   \mathbb{E}_{l_t \sim q_t} \mathbb{E}_{X_t \sim p_t}\left[\sum_{t=1}^T l_t^\top X_t - \min_X \sum_{t=1}^T l_t^\top X  \right] $$
Let $\mathbb{E}_{X_t \sim p_t} = x_t$. 
$$\inf_{p_1 \dots p_T} \sup_{q_1 \dots q_t} \mathbb{E}_{l_t \sim q_t} [\sum_{t=1}^T l_t^\top x_t - \min_X \sum_{t=1}^T l_t^\top X] $$

\LBFull*

\begin{proof}
We choose $q_t$ to be the density such that $l_{t,i}$ is a Rademacher random variable, ie, $l_{t,i} = +1$ w.p. $1/2$ and $l_{t,i}=-1$ w.p $1/2$ for all $t=1\dots T$ and $i=[n]$. So,
\begin{align*}
    &\inf_{p_1 \dots p_T} \sup_{q_1 \dots q_t} \mathbb{E}_{l_t \sim q_t} \left[\sum_{t=1}^T l_t^\top x_t - \min_X \sum_{t=1}^T l_t^\top X   \right] \\&\geq \inf_{p_1 \dots p_T} \mathbb{E}_{l_{t}} \left[\sum_{t=1}^T l_t^\top x_t - \min_X \sum_{t=1}^T l_t^\top X  \right]
\end{align*}
For our choice of $q_t$, we have $\mathbb{E}_{l_{t}} [l_t^\top x_t] = 0$. So,
\begin{align*}
    &\inf_{p_1 \dots p_T} \mathbb{E}_{l_{t}} [\sum_{t=1}^T l_t^\top x_t - \min_X \sum_{t=1}^T l_t^\top X] \\&= \inf_{p_1 \dots p_T} \mathbb{E}_{l_{t}} [- \min_X \sum_{t=1}^T l_t^\top X] \\
    &= \mathbb{E}_{l_{t}} [\max_X \sum_{t=1}^T l_t^\top X]
\end{align*}


Simplifying this, we get:
\begin{align*}
        \mathbb{E}_{l_{t}} [\max_X \sum_{t=1}^T l_t^\top X] &= \mathbb{E}_{l_{t}} [\max_{X_1\dots X_n} \sum_{t=1}^T \sum_{i=1}^n l_{t,i} X_i]\\
        &= \mathbb{E}_{l_{t}}[\sum_{i=1}^n\max_{X_i} \sum_{t=1}^T  l_{t,i} X_i]\\
        &= \sum_{i=1}^n \mathbb{E}_{l_{t,i}}[\max_{X_i} \sum_{t=1}^T  l_{t,i} X_i]\\
        &= n \mathbb{E}_{Y}[\max_{x} \sum_{t=1}^T  Y_{t} x]
\end{align*}
Here $Y$ is a Rademacher random vector of length $T$ and $x \in \{0,1\}$. We have that
$$\max_{x} \left[\sum_{t=1}^T  Y_{t} x\right] =\begin{cases} 0 \quad \text{ If } \sum_{t=1}^T  Y_{t} \leq 0 \\ \sum_{t=1}^T  Y_{t} \quad \text{ otherwise}
\end{cases}$$
So
\begin{align*}
    \mathbb{E}_{Y}\left[\max_{x} \sum_{t=1}^T  Y_{t} x  \right] &= \mathbb{E}_{Y}[\sum_{t=1}^T  Y_{t} | \sum_{t=1}^T  Y_{t} >0]\\
    &= \frac{1}{2}\mathbb{E}_{Y}  \left| {\sum_{t=1}^T  Y_{t}} \right|  
\end{align*}
Using Khintchine's inequality, we have positive constants $A$ and $B$ such that:
$$A\left( \sum _ { t = 1 } ^ { T } \left|1 \right| ^ { 2 } \right) ^ { 1 / 2 } \leq \mathbb{E}_{Y}  \left| {\sum_{t=1}^T  Y_{t}} \right| \leq B\left( \sum _ { t = 1 } ^ { T } \left|1 \right| ^ { 2 } \right) ^ { 1 / 2 }$$
Hence, the regret is lower bounded by $\Omega(n \sqrt{T})$.
\end{proof}
\subsubsection{Bandit Lower bound}
\LBBandit*
\begin{proof}
We consider $2^n$ stochastic adversaries indexed by $X \in \{0,1\}^n$. Adversary $X$ draws losses as follows:
\begin{equation*}
    l_{t,i} = \begin{cases} \begin{cases} +1 \text{ w.p } \frac{1}{2}+\epsilon\\
    -1 \text{ w.p } \frac{1}{2}-\epsilon
    \end{cases} \text{ if } X_i = 0\\
    \begin{cases} +1 \text{ w.p } \frac{1}{2} - \epsilon\\
    -1 \text{ w.p } \frac{1}{2} + \epsilon
    \end{cases} \text{ if } X_i = 1
    \end{cases}
\end{equation*}
Let $\tilde{l}_{t} = [X_1^\top l_1,X_2^\top l_2,\dots,X_t^\top l_t]$. We consider deterministic algorithms, ie $X_t$ is a deterministic function of $\tilde{l}_{t-1}$. So, the only the adversary's randomness remains. The obtained result can be extended to randomized algorithms via application of Fubini's Theorem. Let $E_X$ denote the expectation conditioned on adversary $X$. When playing against adversary $X$, the vector $X$ is the best action in expectation. The expected regret when playing against adversary $X$.
\begin{align*}
    \mathbb{E}_X[\mathcal{R}_T] &= \mathbb{E}_X \left[ \sum_{t=1}^T l_t^\top X_t - \min_{X^\star}\sum_{t=1}^T l_t^\top X^\star\right]\\
    &\geq \mathbb{E}_X \left[ \sum_{t=1}^T l_t^\top X_t - \sum_{t=1}^T l_t^\top X\right]\\
    &= 2\epsilon \sum_{i=1}^n \mathbb{E}_X[\sum_{t=1}^T \textbf{1}(X_{i,t} \neq X_i)]\\
    &= 2\epsilon T \sum_{i=1}^n \left(1- \frac{\mathbb{E}_X[\sum_{t=1}^T \textbf{1}(X_{i,t} = X_i)]}{T} \right)
\end{align*}
$\sum_{t=1}^T \textbf{1}(X_{i,t} = X_i)/T$ is the empirical mean of playing $X_i$. Let $J_i$ be a Bernoulli random drawn according to this mean. Hence,
$$\mathbb{E}_X[\mathcal{R}_T] \geq 2\epsilon T \sum_{i=1}^n \left(1- \mathbb{P}_X(J_i=X_i) \right)$$
Taking the average over adversaries:
\begin{align*}
    \mathbb{E}[\mathcal{R}_T] &= \frac{1}{2^n}\sum_{X} \mathbb{E}_X[\mathcal{R}_T]\\
    &\geq 2\epsilon T \sum_{i=1}^n \left(1- \frac{1}{2^n}\sum_{X}\mathbb{P}_X(J_i=X_i) \right)
\end{align*}
Let $X^{\oplus i}$ be the vector $X$ with the $i$'th bit flipped. Using Pinsker's inequality, we have that:
$$\mathbb{P}_X(J_i = X_i) \leq \mathbb{P}_{X^{\oplus i}}(J_i = X_i) + \sqrt{\frac{1}{2}KL(\mathbb{P}_{X^{\oplus i}}\| \mathbb{P}_X)}$$
Taking the summation, and using the concavity of square root:
$$\frac{1}{2^n}\sum_{X} \mathbb{P}_X(J_i = X_i) \leq \frac{1}{2} + \sqrt{\frac{1}{2}\frac{1}{2^n}\sum_{X}KL(\mathbb{P}_{X^{\oplus i}}\| \mathbb{P}_X)}$$

The sequence of observed losses $\tilde{l}_{T} \in \{-n,\dots,+n\}^T$ determines the empirical distribution of plays. Let $\mathbb{P}^T_X$ be the law of $\tilde{l}_{T}$ when playing against adversary $X$. So, using the chain rule of Kullback Leibler divergence:
\begin{align*}
    &KL(\mathbb{P}_{X^{\oplus i}}\| \mathbb{P}_X)\leq KL(\mathbb{P}^T_{X^{\oplus i}}\| \mathbb{P}^T_X)  \\
    &=KL(\mathbb{P}^1_{X^{\oplus i}}\| \mathbb{P}^1_X) \\&+ \sum _ { t = 2 } ^ { T } \sum_{ \tilde{l} _ {t - 1 }  } \mathbb{P}^{t-1}_{X^{\oplus i}}(\tilde{l} _ { t - 1 })  KL(\mathbb{P}^t_{X^{\oplus i}}(\cdot|\tilde{l} _ { t - 1 })\| \mathbb{P}^t_X((\cdot|\tilde{l} _ {t - 1 }))\\
    &= KL(\mathcal{B}_{0}\|\mathcal{B'}_0) \textbf{1}(X_{1,i} = X_i) \\
    &+  \sum _ { t = T } ^ { t } \sum_{ \tilde{l} _ {t - 1 }:X_{t,i} = X_i  } \mathbb{P}^{t-1}_{X^{\oplus i}}(\tilde{l} _ { t - 1 })KL(\mathcal{B}_{\tilde{l}_{t-1}}\|\mathcal{B'}_{\tilde{l}_{t-1}})
\end{align*}
Here, $\mathcal{B}_{\tilde{l}_{t-1}},\mathcal{B'}_{\tilde{l}_{t-1}}$ are sums of at most $n$ Bernoulli random variables such that their means agree on all coordinates except $i$.
Using Lemma 24 from \cite{audibert2011minimax}, we get that:
$$KL(\mathcal{B}_{\tilde{l}_{t-1}}\|\mathcal{B'}_{\tilde{l}_{t-1}}) \leq \frac{16\epsilon^2}{ n }$$
Substituting this back into the previous expression, we get:
\begin{align*}
    KL(\mathbb{P}_{X^{\oplus i}}\| \mathbb{P}_X) &\leq \frac{16\epsilon^2}{n} \sum_{t=1}^T \sum_{\tilde{l}_{1:t-1} : X_{t,i}=X_i}\mathbb{P}^t_{X^{\oplus i}}(\tilde{l}_{1:t-1})\\
    &\leq \frac{16\epsilon^2}{n} \sum_{t=1}^T \mathbb{E}_{X^{\oplus i}}(\textbf{1}(X_{i,t}=X_i))\\
    &= \frac{16\epsilon^2}{n} T \mathbb{P}_{X^{\oplus i}}(J_i = X_i)
\end{align*}
Taking the summation, we have:
\begin{align*}
    \frac{1}{2^n} \sum_X KL(\mathbb{P}_{X^{\oplus i}}\| \mathbb{P}_X) \leq \frac{8\epsilon^2}{n} T 
\end{align*}
Substituting this in the regret inequality:
\begin{align*}
    \mathbb{E}[\mathcal{R}_T]&\geq 2\epsilon T \sum_{i=1}^n \left( 1- \frac{1}{2} - \sqrt{\frac{4 \epsilon^2 T}{n}}\right)\\
    &= 2\epsilon T n \left(\frac{1}{2} - 2 \epsilon\sqrt{\frac{T}{n}}\right)
\end{align*}
Optimizing over $\epsilon$, we get that $\mathbb{E}[\mathcal{R}_T] = \Omega(n^{3/2}\sqrt{T})$
\end{proof}

\subsection{$\{-1,+1\}^n$ Hypercube Case}
\begin{lemma} \label{lemma6}Exp2 on $\{-1,+1\}^n$ with losses $l_t$ is equivalent to Exp2 on $\{0,1\}^n$ with losses $2l_t$ while using the map $2X_t-\textbf{1}$ to play on $\{-1,+1\}^n$.
\end{lemma}
\begin{proof}
Consider the update equation for Exp2 on $\{-1,+1\}^n$
$$p_{t+1}(Z) = \frac{\exp(-\eta \sum_{\tau=1}^t Z^\top l_\tau)}{\sum_{W \in \{-1,+1\}^n}\exp(-\eta \sum_{\tau=1}^t W^\top l_\tau)}$$
$Z \in \{-1,+1\}^n$ can be mapped to a $X \in \{0,1\}^n$ using the bijective map $X = (Z+\textbf{1})/2$. So:
\begin{align*}
p_{t+1}(Z) &= \frac{\exp(-\eta \sum_{\tau=1}^t (2X-\textbf{1})^\top l_\tau)}{\sum_{Y \in \{0,1\}^n}\exp(-\eta \sum_{\tau=1}^t (2Y-\textbf{1})^\top l_\tau)}\\
&= \frac{\exp(-\eta \sum_{\tau=1}^t X^\top (2l_\tau))}{\sum_{Y \in \{0,1\}^n}\exp(-\eta \sum_{\tau=1}^t Y^\top (2l_\tau))}
\end{align*}
This is equivalent to updating the Exp2 on $\{0,1\}^n$ with the loss vector $2l_t$.
\end{proof}
\Hypereq*
\begin{proof}
After sampling $X_t$, we play $Z_t = 2X_t-\textbf{1}$. So $\Pr(X_t=X) = \Pr(Z_t = 2X -\textbf{1})$. In full information, $2\tilde{l}_t = 2l_t$ and in the bandit case $\mathbb{E}[2\tilde{l}_t] = 2l_t$. Since $2\tilde{l}_t$ is used to update the algorithm, by Lemma \ref{lemma6} we have that $\Pr(X_{t+1}=X) = \Pr(Z_{t+1} = 2X -\textbf{1})$. By equivalence of Exp2 to PolyExp, the first statement follows immediately. Let $Z^\star = \min \limits_{Z \in \{-1,+1\}^n} \sum_{t=1}^T Z^\top l_t$ and $2X^\star = Z^\star + \textbf{1}$. The regret of Exp2 on $\{-1,+1\}^n$ is:
\begin{align*}
\sum_{t=1}^T l_t^\top (Z_t - Z^\star) &= \sum_{t=1}^T l_t^\top (2X_t -\textbf{1} - 2X^\star + \textbf{1})\\&= \sum_{t=1}^T (2l_t)^\top (X_t - X^\star)
\end{align*}
\end{proof}

